Group-disentangled Representation Learning with Weakly-Supervised Regularization

Learning interpretable and human-controllable representations that uncover factors of variation in data remains an ongoing key challenge in representation learning. We investigate learning group-disentangled representations for groups of factors with weak supervision. Existing techniques to address this challenge merely constrain the approximate posterior by averaging over observations of a shared group. As a result, observations with a common set of variations are encoded to distinct latent representations, reducing their capacity to disentangle and generalize to downstream tasks. In contrast to previous works, we propose GroupVAE, a simple yet effective Kullback-Leibler (KL) divergence-based regularization across shared latent representations to enforce consistent and disentangled representations. We conduct a thorough evaluation and demonstrate that our GroupVAE significantly improves group disentanglement. Further, we demonstrate that learning group-disentangled representations improve upon downstream tasks, including fair classification and 3D shape-related tasks such as reconstruction, classification, and transfer learning, and is competitive to supervised methods.

==> figures/groupvae/tikz/unsupervised.tex <==
\begin{tikzpicture}[
        % >=stealth, % arrow head style
        shorten > = 1pt, % don't touch arrow head to node
        auto,
        node distance = 2cm, % distance between nodes
        semithick % line style
        ]
        \tikzstyle{every state}=[
            draw=black,
            thick,
            fill=white,
            minimum size=8mm
        ]
        \node[state,fill=gray!30] at (0, 0) (x) {$x$};
        \node[state] (z) at (0, 1.75) {$z$};
        \draw[->] (z) -- (x);
\end{tikzpicture}

==> figures/groupvae/tikz/weakly_supervised.tex <==
\begin{tikzpicture}[
    >=stealth, % arrow head style
    shorten > = 1pt, % don't touch arrow head to node
    auto,
    node distance = 2cm, % distance between nodes
    semithick % line style
    ]
    \tikzstyle{every state}=[
        draw=black,
        thick,
        fill=white,
        minimum size=8mm
    ]
    \node[state,fill=gray!30,minimum size=1cm] at (0.75, 0) (x) {$x$};
    \node[state,fill=gray!30,minimum size=1cm] at (2.25, 0) (xp) {$x'$};
    \node[state,minimum size=1cm] (zs) at (0, 1.75) {$z_{\backslash c}$};
    \node[state,minimum size=1cm] (zg) at (1.5, 1.75) {$\bar{z}_{c, c'}$};
    \node[state,minimum size=1cm] (zsp) at (3., 1.75) {$z_{\backslash c'}$};
    \draw[->] (zs) -- (x);
    \draw[->] (zg) -- (x);
    \draw[->] (zg) -- (xp);
    \draw[->] (zsp) -- (xp);
    % \draw[dashed,<->] (zs.north) to[bend left=55] (zg.north);
    % \draw[dashed,<->] (zg.north) to[bend left=55] (zsp.north);
\end{tikzpicture}
